Block Krylov subspace recycling for shifted systems with unrelated right-hand sides

Many Krylov subspace methods for shifted linear systems take advantage of the invariance of the Krylov subspace under a shift of the matrix. However, exploiting this fact in the non-Hermitian case introduces restrictions; e.g., initial residuals must be collinear and this collinearity must be maintained at restart. Thus we cannot simultaneously solve shifted systems with unrelated right-hand sides using this strategy, and all shifted residuals cannot be simultaneously minimized over a Krylov subspace such that collinearity is maintained. It has been shown that this renders them generally incompatible with techniques of subspace recycling [Soodhalter et al. APNUM '14]. This problem, however, can be overcome. By interpreting a family of shifted systems as one Sylvester equation, we can take advantage of the known "shift invariance" of the Krylov subspace generated by the Sylvester operator. Thus we can simultaneously solve all systems over one block Krylov subspace using FOM or GMRES type methods, even when they have unrelated right-hand sides. Because residual collinearity is no longer a requirement at restart, these methods are fully compatible with subspace recycling techniques. Furthermore, we realize the benefits of block sparse matrix operations which arise in the context of high-performance computing applications. In this paper, we discuss exploiting this Sylvester equation point of view which has yielded methods for shifted systems which are compatible with unrelated right-hand sides. From this, we propose a recycled GMRES method for simultaneous solution of shifted systems.Numerical experiments demonstrate the effectiveness of the methods.

==> figures/BlocksGMRES_2normConverge.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/BlocksGMRES_2normConverge.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between shifted block GMRES 
method and the method of Frommer and Gl\"assner 
for restart parameter $m=40$\label{figure.BlocksGMRES_2normConverge}}
\end{figure}



==> figures/FourAlgCompare.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/FourAlgCompare.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between shifted block GMRES 
method and the method of Frommer and Gl\"assner 
for restart parameter $m=40$\label{figure.FourAlgCompare}}
\end{figure}



==> figures/diffRHSSeqCompare.tex <==

\begin{table}[htb]
\caption{Comparison of block sFOM and block sGMRES with their sequentially applied counterparts when each initial residuals of the shifted systems are not collinear for one matrix from {\tt Group 2}. Both in terms of iteration counts and when multiplying block iterations by the ratio of block matvec cost to single matvec cost, we see that our proposed methods outperform their single-vector counterparts.}
\label{table.diffRHSSeqCompare}
\begin{center}
\begin{tabular}{c|c|c}
Method & Matvecs & Block Matvecs $\times 3.3$ \\
\hline
Shifted Block GMRES & 525 & 1732 \\
Sequential GMRES & 2836 & * \\
Shifted Block FOM & 602 & 1987 \\
Sequential FOM & 3126 & * \\
\end{tabular}
\end{center}
\end{table}



==> figures/fourMethodCompare.tex <==

\begin{table}[htb]
\caption{Comparison of Algorithms \ref{alg.shbl-gmres} and \ref{alg.shbl-fom} with the shifted GMRES method of Frommer and Gl\"assner and the shifted FOM method of Simoncini for four matrices from {\tt Group 2}.  For three of the matrices, the proposed methods yield improved matvec counts, but greater costs when the block matrix-vector product cost muliplier is used. This ratio will be different for different matrices and in different computing environments. The other matrices not show yielded similar results. }
\label{table.fourMethodCompare}
\begin{center}
\begin{tabular}{c|c|c|c|c}
Method & Matrix 1 & Matrix 2 & Matrix 3 & Matrix 4 \\
\hline
Sh. Bl. GMRES (mv $\times 3.3$) & 602\ (2408) & 1759\ (5805) & 634\ (2092) & 555\ (1832) \\
sGMRES & 938 & 1090 & 665 & 597 \\
Sh. Bl. FOM (mv $\times 3.3$) & 982\ (3241) & 1195\ (3944) & 742\ (2449) & 733\ (2419) \\
sFOM & 1177 & 1242 & 756 & 882 \\
\end{tabular}
\end{center}
\end{table}



==> figures/fourMethodCompareRandAnfang.tex <==

\begin{table}[htb]
\caption{Comparison of Algorithms \ref{alg.shbl-gmres} and \ref{alg.shbl-fom} with the shifted GMRES method of Frommer and Gl\"assner and the shifted FOM method of Simoncini for four matrices from {\tt Group 2}.  For three of the matrices, the proposed methods yield improved matvec counts, but greater costs when the block matrix-vector product cost muliplier is used. This ratio will be different for different matrices and in different computing environments. The other matrices not show yielded similar results. }
\label{table.fourMethodCompareRandAnfang}
\begin{center}
\begin{tabular}{c|c|c|c|c}
Method & Matrix 1 & Matrix 2 & Matrix 3 & Matrix 4 \\
\hline
Sh. Bl. GMRES (mv $\times 3.3$) & 628\ (2512) & 1759\ (5805) & 634\ (2092) & 555\ (1832) \\
sGMRES & 938 & 1090 & 665 & 597 \\
Sh. Bl. FOM (mv $\times 3.3$) & 959\ (3165) & 1195\ (3944) & 742\ (2449) & 733\ (2419) \\
sFOM & 1177 & 1242 & 756 & 882 \\
\end{tabular}
\end{center}
\end{table}



==> figures/shblDiffRestParam.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shblDiffRestParam.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Demonstration of block shifted GMRES behavior for various restart parameters, 
where darker lines indicate longer restart cycles\label{figure.shblDiffRestParam}}
\end{figure}



==> figures/shblFOMFrommerCompare.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shblFOMFrommerCompare.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between shifted block GMRES 
method and the method of Frommer and Gl\"assner 
for restart parameter $m=40$\label{figure.shblFOMFrommerCompare}}
\end{figure}



==> figures/shblFOM_GMRESCompare.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shblFOM_GMRESCompare.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between shifted block GMRES 
method and shifted block FOM 
for restart parameter $m=40$ and twelve shifts for the fourth matrix from {\tt Group 1}.We began with collinear residuals (same right hand side and all zero initial approximations)
\label{figure.shblFOM_GMRESCompare}}
\end{figure}



==> figures/shblFOM_sFomSimonciniCompare.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shblFOM_sFomSimonciniCompare.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between shifted block FOM 
method and the method of Simoncini 
for restart parameter $m=40$ and twelve shifts for the fourth matrix from {\tt Group 1}.We began with collinear residuals (same right hand side and all zero initial approximations)
\label{figure.shblFOM_sFomSimonciniCompare}}
\end{figure}



==> figures/shblFrommerCompare.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shblFrommerCompare.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{Convergence comparison between sbGMRES 
method and sGMRES \cite{Frommer1998} 
for restart parameter $m=40$ and twelve shifts for the fourth matrix from {\tt Group 1}.We began with collinear residuals (same right hand side and all zero initial approximations)
\label{figure.shblFrommerCompare}}
\end{figure}



==> figures/shiftedStagToy.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shiftedStagToy.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{\label{figure.shiftedStagToy} Relative two-norm residual curves for stagnating  shifted block GMRES and shifed block FOM for the $30\times 30$ shift matrix. The black solid and dashed curves correspond respectively to the  block shifted FOM and GMRES residuals for the base system.  Similarly,  the gray solid and dashed curves, respectively, correspond to the shifted system.}
\end{figure}



==> figures/shiftedStagToyDefl.tex <==

\begin{figure}[htb]
\hfill
\includegraphics[scale=0.35]{figures/shiftedStagToyDefl.eps}
\hfill
\begin{picture}(0,0)
\end{picture}
\caption{\label{figure.shiftedStagToyDefl} Relative two-norm residual curves for stagnating  shifted block GMRES and shifed block FOM for the $30\times 30$ shift matrix  with with a base system and two shifted systems.  The right-hand sides are chosen so that a linear dependent  Arnoldi vector will be generated and replaced at iteration $5$.  The black solid and dashed curves correspond respectively to the  block shifted FOM and GMRES residuals for the base system.  Similarly,  the dark gray solid and dashed curves, respectively, correspond to the first shifted system with $\sigma=1$.  The light gray solid and dashed curves correspond to the second shifted system with $\sigma=2$.}
\end{figure}


